In-Application Defense Against Evasive Web Scans through Behavioral Analysis

Web traffic has evolved to include both human users and automated agents, ranging from benign web crawlers to adversarial scanners such as those capable of credential stuffing, command injection, and account hijacking at the web scale. The estimated financial costs of these adversarial activities are estimated to exceed tens of billions of dollars in 2023. In this work, we introduce WebGuard, a low-overhead in-application forensics engine, to enable robust identification and monitoring of automated web scanners, and help mitigate the associated security risks. WebGuard focuses on the following design criteria: (i) integration into web applications without any changes to the underlying software components or infrastructure, (ii) minimal communication overhead, (iii) capability for real-time detection, e.g., within hundreds of milliseconds, and (iv) attribution capability to identify new behavioral patterns and detect emerging agent categories. To this end, we have equipped WebGuard with multi-modal behavioral monitoring mechanisms, such as monitoring spatio-temporal data and browser events. We also design supervised and unsupervised learning architectures for real-time detection and offline attribution of human and automated agents, respectively. Information theoretic analysis and empirical evaluations are provided to show that multi-modal data analysis, as opposed to uni-modal analysis which relies solely on mouse movement dynamics, significantly improves time-to-detection and attribution accuracy. Various numerical evaluations using real-world data collected via WebGuard are provided achieving high accuracy in hundreds of milliseconds, with a communication overhead below 10 KB per second.

==> 08-Related.tex <==
\section{Related Work}
\label{sec:related_work}
\ak{this will be updated}
%\subsection{Current Defense Solutions}
We focus on three main layers of defense against automated web traffic. We explain each layer and discuss their effectiveness and potential weaknesses. 

% Furthermore, we shortly describe the recent overview of the methods evading the contemporary defenses.

\noindent \textbf{The Role of Fingerprinting.} Conventional fingerprinting techniques~\cite{10.5555, NikiforakisKJKPV13, laperdrix2020browser, zhang2022survey} gather specific details about connecting devices such as user agents, hardware details, geolocation, and generate a unique id for that device. Fingerprints can be used for several purposes such as detecting previously seen adversarial agents attempting to visit the target web application. If an agent with automated activity is detected, the corresponding fingerprint will be used in subsequent checks. While fingerprinting mechanisms have been useful in tracking real users, they offer limited capabilities to identify modern evasive attacks. In particular, it is not very difficult to generate malicious code that can report any arbitrary identity or establish connections from different parts of the web while launching attacks in a stealthy way~\cite{webbot,6575366,phishlab} -- as mentioned in the threat model. For instance, it is very common to incorporate various network proxies and use less suspicious traffic sources, use full-fledged browsers instead of using curl or headless browsers, and report arbitrary information while interacting with the web application, making the current defense mechanisms less effective in detecting more evasive cases. 

\noindent \textbf{Challenge-based Defense Systems.} The predominant category of challenge-based defense systems revolves around CAPTCHAs challenges. Notable CAPTCHA tools widely employed encompass Image-based CAPTCHA, reCAPTCHA \cite{von2004telling, von2008recaptcha}, reCAPTCHA v2~\cite{google-recaptcha}, and hCAPTCHA~\cite{hcaptcha}. Although CAPTCHAs exhibit efficacy, they are susceptible to circumvention through advanced techniques. In the realm of image-based CAPTCHAs, a breakthrough attack is proposed by the authors of \cite{alqahtani2020image}. Furthermore, in the landscape of text-based CAPTCHAs, innovative attacks have been introduced by the authors of \cite{george2017generative} and \cite{bursztein2014end}, leveraging generative segmentation of characters without specific heuristics, thereby enhancing the methods' generalizability. Other studies, such as \cite{bock2017uncaptcha}, \cite{aiken2018poster}, and \cite{sano2013solving}, delve into the deciphering of audio-based CAPTCHAs. 

\noindent \textbf{Behavior Analysis and Machine Learning}. Recent advances propose the analysis of user behavior to identify patterns associated with automated attacks. User behavior is reflected in multiple aspects both on the server and client sides. Several studies including \cite{suchacka2021efficient, tanaka2020bot} have proposed different methods for analyzing HTTP requests on the server side using machine learning algorithms. Conversely, the client side is imprinted with the footsteps of visitors. Several research studies including \cite{niu2023exploring, wei2019deep } have proposed methods for analyzing the mouse movements of visitors in order to distinguish bots from humans. Additionally, authors of \cite{iliou2021detection} have combined the analysis of mouse movements together with the HTTP logs to develop a framework for bot detection. We have shown that including other browser events can increase the accuracy of detection while making it harder for adversaries to replicate human behavior. Furthermore, analysis of touch events can lead to a uniform solution for mobile and desktop platforms.

% \noindent \textbf{Evading the Defenses.} As defenders employ sophisticated tools such as device fingerprinting, CAPTCHA challenges, and behavioral analysis, adversaries respond with equally sophisticated evasion techniques. Attackers may employ tactics to manipulate or mimic legitimate device characteristics, rendering device fingerprinting less effective. CAPTCHA challenges, designed to thwart automated bots, face evasion attempts through the use of advanced bots or by outsourcing the solving process to human operators. Furthermore, attackers continually refine their strategies to mimic human-like behavior, presenting a formidable challenge for machine learning models engaged in behavioral analysis. The evasion side thus underscores the dynamic nature of cybersecurity, urging defenders to remain vigilant and adapt their approaches to stay ahead of evolving threats.
